The Sample Complexity of Smooth Boosting and the Tightness of the Hardcore Theorem

Smooth boosters generate distributions that do not place too much weight on any given example. Originally introduced for their noise-tolerant properties, such boosters have also found applications in differential privacy, reproducibility, and quantum learning theory. We study and settle the sample complexity of smooth boosting: we exhibit a class that can be weak learned to $\gamma$-advantage over smooth distributions with $m$ samples, for which strong learning over the uniform distribution requires $\tilde{\Omega}(1/\gamma^2)\cdot m$ samples. This matches the overhead of existing smooth boosters and provides the first separation from the setting of distribution-independent boosting, for which the corresponding overhead is $O(1/\gamma)$. Our work also sheds new light on Impagliazzo's hardcore theorem from complexity theory, all known proofs of which can be cast in the framework of smooth boosting. For a function $f$ that is mildly hard against size-$s$ circuits, the hardcore theorem provides a set of inputs on which $f$ is extremely hard against size-$s'$ circuits. A downside of this important result is the loss in circuit size, i.e. that $s' \ll s$. Answering a question of Trevisan, we show that this size loss is necessary and in fact, the parameters achieved by known proofs are the best possible.

==> BoostingReferences.tex <==
\section{Applications to Boosting}
\subsection{Setup}

\begin{definition}[$\eps$-weak learner]
    A learning algorithm $A$ is a $\eps$-weak learner for a target class $\mcC$ if for all $c \in \mcC$, and for all distributions $\mcD$ over the domain $\mcX$, if given $\delta > 0i$ and $m \geq m_\mcC(\delta)$ i.i.d. examples generated by $\mcD$, the algorithm will return a hypothesis $h$ such that, with probability at least $1-\delta$, $L_{\mcD}(h) \leq \frac{1}{2} - \eps$.

    $\eps$ is called $A$'s edge.
\end{definition}
Note: one difference with the setup we have been considering is that weak learners here are allowed to fail with probability $\delta$.

\begin{definition}
    A boosting algorithm $B$ is given access to an $\eps$-weak PAC learning algorithm $A$ for $\mcC$ as well as $m = m(\eps, \delta)$ examples labeled according to any $c \in \mcC$, and drawn according to any distribution $\mcD$ will return a hypothesis $H$ such that $L_\mcD(H) \leq \eps$ w.p. at least $1 - \delta$.
\end{definition}

\begin{remark}[Some requirements on $B$] $ $\newline
    \begin{enumerate}
        \item ``A boosting algorithm should be general in the sense of not requiring knowledge of the target class $\mcC$''
        \item $B$'s sample size $m$ should be polynomial in its parameters.
        \item No other restrictions on $B$, it could have superpolynomial running time, or output a combined hypothesis of any form.
    \end{enumerate}
\end{remark}

\subsection{Lower-bounding the number of rounds}

\begin{theorem}
    Let $B$ be any boosting algorithm as defined above, $0 < \eps < \frac{1}{2}$. Then for any $\nu > 0$, there exists a target class $\mcC$, a distribution $\mcD$, a target function $c \in \mcC$, and an $\eps$-weak learning algorithm $A$ such that if $B$ makes $T$ calls to $A$, then the generalization error of its combined classifier will be at least:
    $$\mathrm{Binom} \left ( T, \frac{T}{2}, \frac{1}{2} + \eps \right ) - \nu$$
    with probability at least $1 - \nu$.
\end{theorem}

Notes: this means that if we require $B$ to have its confidence parameter $\delta < \nu$ then its error parameter $\eps$ cannot be made smaller without increasing $T$.

The matching upper bound is given by the Boost By Majority algorithm.

\textit{Proof sketch.}
The target class $\mcC$ is constructed by first selecting a random function $c: \mcX \rightarrow \bits$ by independently, for each $x \in \mcX$, choosing $c(x)$ to be $-1$ or $+1$ with equal probability. The class $\mcC$ is then chosen to consist of this single function $\mcC = \{c\}$.

The proof then uses oblivious weak learners that randomly choose a hypothesis $h$ such that, for each $x$, $h(x)$ is chosen randomly to be $c(x)$ w.p. $\frac{1}{2} + \eps$ and $-c(x)$ otherwise.

Crucially, the proof uses the fact that the boosting algorithm does not know $\mcC$ (even though the weak learner does) or else the target $c$ could be learned with no data.


\subsection{Lower-bounding the sample complexity of the booster}

\begin{theorem} [\cite{larsen2022optimal}]
    For all $d \in \mathbb{N}$ and every $2^{-d} < \gamma < 1/80$, there is a finite set $\mathcal{X}$, a concept class $\mcC \subseteq \mcX \rightarrow \bits$, and a hypothesis set $\mcH \subseteq \mcX \rightarrow \bits$ of VC-dimension at most $d$, such that for every $(\eps, \delta)$ with $0 < \eps < 1$ and $0 < \delta < 1/3$, there is a distribution $\mcD$ over $\mcX$ such that:
    \begin{enumerate}
        \item For every $c \in \mcC$ and every distribution $\mcD'$ over $\mcX$, there is an $h \in \mcH$ with $\Pr_{x \sim \mcD'}[h(x) \neq c(x)] \leq 1/2 - \gamma$. (i.e. $\mcC$ can be weakly learned).
        \item For any algorithm $A$, there is a concept $c \in \mcC$ such that $A$ requires 
        $$\Omega \left (\frac{d}{\eps \gamma^2} + \frac{\log(1/\delta)}{\eps}\right )$$
        samples $S$ to guarantee $L_\mcD(h_S) \leq \eps$ with probability at least $1 - \delta$.
    \end{enumerate}
\end{theorem} 
\begin{remark}
    The lower bound does not require the algorithm to even use a $\gamma$-weak learner, nor does it need to run in polynomial time. It is also allowed to use the full knowledge of the set $\mcC$ and the distribution $\mcD$. The only thing it does not know is which concept $c \in \mcC$ provides the labels to the training samples.
\end{remark}

\textit{Proof sketch.} The $\frac{\log(1/\delta)}{\eps}$ term comes from previous work on tight lower-bounds for PAC-learning in the realizable setting (obtained by setting $\mcC = \mcH$).

The hypothesis set $\mcH$ is defined over a domain $\mcX = (x_1, \dots, x_u)$ with $u = O(d \gamma^-2)$ such that a constant fraction of all concepts in $\mcX \rightarrow \bits$ can be $\gamma$-weakly learned from $\mcH$. The concept class $\mcC$ is the set of all labelings on $\mcC$. The hard distribution $\mcD$ is samples $x_1$ with probability $1 - u/(4m)$ and with the remaining probability samples uniformly among $x_2, \dots, x_u$. The key is that we only expect to see $1 + u/4$ distinct points from $\mcX$ in a sample $S$ of cardinality $m$. Thus if the weak learner returns a random concept, the labels it assigns to points in $\mcX \setminus S$ are almost uniform random and independent and the best any algorithm $\mcA$ can do is just guess.
If we condition on receiving a sample other than $x_1$ (this happens with probability $O(d \gamma^-2/m)$), the algorithm will thus fail with constant probability.

The proof then proceeds by showing that a random concept $c \in \mcC$, the entropy of $c$ is high, even conditioned on $S$ and the labels $c(S)$ but $A(S)$ is a function of $S$ and $c(S)$ hence $A(S)$ cannot have small error probability under $\mcD$.

\section{Sample complexity of smooth boosting}

\subsection{Background and definitions}
\begin{definition}[$\kappa$-smooth distribution]
    A distribution $\mcD$ is $\kappa$-smooth if $\|2^n\mcD\|_\infty \leq \kappa$. 
\end{definition}
This notion of smoothness relies on the fact that no element has too much weight. (Equivalently, the distribution has high minimum entropy $\log(\|\mcD\|_\infty^{-1})$). It is also similar to dominated distributions in average-case complexity.
\begin{definition}[Smooth boosting]
    A \emph{smooth boosting algorithm} $B$ is given access to a $\gamma$-weak PAC learning algorithm $A$ for the concept class $C$ and $m = m(\eps, \delta, \gamma)$ examples labeled according to any $c \in \mcC$ and drawn according to any smooth distribution $\mcD$. By only querying the weak learner with smooth distribution, $B$ returns a hypothesis $H$ such that $L_\mcD(H) \leq \eps$ with probability at least $1 - \delta$.
\end{definition}

\begin{remark}
I'm not sure if the $\mcD$ has to be smooth for this definition. In fact, it seems to depend on the model of boosting we are using.
    \begin{itemize}
        \item In the original boosting and hardcore set construction paper \cite{boosting_hardcore_set}, the booster has access to an example oracle $\EX(f, \mcD)$ which, when queried, provides a labelled example $\langle x, f(x) \rangle$ where $x$ is drawn according to $\mcD$ and $f$ is the unknown target function. Since the first call to the example oracle is done with the original distribution $\mcD$, then we would require $\mcD$ to be smooth. This is called \textbf{boosting-by-filtering}.
        \item In the Smooth Boosting and Learning with Malicious Noise paper \cite{smooth_boosting_with_noise}, the boosting algorithm is given access to a dataset of labeled examples then generates (smooth) probability distributions over the dataset to give to the weak learner. Proofs then show that the generalization error is low given hypotheses of bounded VC-dimension and sufficiently large training sets. Boosting algorithms that work with a fixed sample are called \textbf{boosting-by-sampling} algorithms. In this case, the original distribution $\mcD$ (on the domain) does not seem to have to be smooth.
    \end{itemize}
I do not think this is a major issue. Both definitions make sense, the first one seems more appropriate to hardcore set construction. This may however be something we should be careful about in phrasing.
\end{remark}
\begin{lemma}[\cite{boosting_simple_learners}, footnote 2 / the Fundamental Theorem of PAC learning] 
\label{lemma:fundamental_theorem_pac}
The sample complexity of (strongly) PAC learning a concept class $\mcC$ of VC-dimension $d$ is $\Tilde{O} \left ( \frac{d + \log ( 1 / \delta)}{\eps} \right )$
\end{lemma}

Note: I'm unsure about the first sentence in the footnote.

\subsection{References on boosting}

\paragraph{Hardcore set constructions yield smooth boosting algorithms \cite{boosting_hardcore_set}} Presents the relationship between hardcore set constructions and smooth boosting algorithms. The relationship goes in both directions; they use the original hardcore set construction by Impagliazzo to create a smooth boosting algorithm (note: boosting algorithms Adaboost are not known to be smooth). Conversely, they use known smooth boosting algorithms to improve the size parameter in the hardcore set construction to $O \left (\frac{\eps^2}{\log(1/\delta)} \right )$.

\paragraph{Smooth boosting and Learning with Malicious Noise \cite{smooth_boosting_with_noise}} An adversary can arbitrarily modify the values of a certain number of samples in the training set. The goal is to boost a noise resistant weak learner into a noise resistant strong learner. Intuitively, the connection with smooth boosting comes from the fact that if the booster does not use a smooth distribution, it could add a lot of weight on an input which is incorrectly labeled (even though the noise rate is low); this cannot happen is the distribution is smooth. Their algorithm $\textsc{SmoothBoost}$ requires $T = O \left ( \frac{1}{\delta \gamma^2 \sqrt{1 - \gamma}} \right )$ rounds which is worse than AdaBoost's $T = O \left ( \frac{\log (1 / \delta)}{\gamma^2} \right )$. The distributions constructed by $\textsc{SmoothBoost}$ satisfy $\|\mcD\|_\infty \leq \frac{1}{\delta m}$ (this is optimal up to constant factors.)

\paragraph{Boosting Simple Learners \cite{boosting_simple_learners}}
They show that if we assume that the boosting algorithm has access to a predetermined (but unknown) class of weak learners that output hypotheses from a \emph{constant} VC-dimension hypothesis class, then the lower bound on oracle complexity (the number of calls to the weak learner) given by Schapire and Freund can be circumvented. In particular, their method only requires $\Tilde{O} \left ( \frac{1}{\gamma}\right ) $ oracle calls instead of $\Tilde{O} \left ( \frac{1}{\gamma^2}\right )$. More specifically, with probability $1 - \delta$, the following happens
\begin{enumerate}
    \item \textbf{Oracle Complexity}: The number of times the weak learner is called satisfies $$T = O \left ( \frac{\log m + \log(1/\delta)}{\gamma}\right )$$
    ($m$ is the number of given samples)
    \item \textbf{Sample Complexity}: The hypothesis $h$ outputted by their algorithm satisfies $\corr_\mcD(h) \geq 1 - \eps$ and the sample complexity $m$ is given by:
    $$m = \Tilde{O} \left ( \frac{1}{\eps} \cdot \left (\frac{m_0}{\gamma} + \frac{1}{\gamma^{d^*}}\right ) \right )$$ where $m_0$ is the sample complexity of the base learners, and $d^*$ is the dual VC-dimension of the base class (if the base class has constant VC-dimension then its dual VC-dimension is also constant.)
\end{enumerate}
\begin{remark}
Note that the dependence on $\frac{1}{\gamma}$ matches the bound given by \Cref{lemma:fundamental_theorem_pac}.
\end{remark}

\paragraph{Applications to differential privacy \cite{privacy_boosting}} Informally, a (randomized) learning algorithm is differentially private if the distribution on hypotheses it produces does not depend too much on any one of its input samples. It is natural to design ``private boosting'' algorithms that transform differentially private weak learners into differentially private strong learners. In this context, smoothness is important for ensuring that each weighted input sample does not have too much of an effect on the outcomes of any of the runs of the weak learner.

\paragraph{Applications to reproducible algorithms \cite{reproducible_learning}} A reproducible learning algorithm is resilient to variations in its samples — with high probability, it returns the exact same output when run on two samples from the same underlying distribution. Again, smooth boosting is important here to ensure that each input sample does not have too much of an effect on any of the outcomes of any of the runs of the weak learner (and hence on the final hypothesis).

\paragraph{Distribution-specific agnostic boosting \cite{kanade2009:potential, feldman2009:distribution}} The work in this area focuses on boosting algorithms that are distribution-specific i.e. the weak learner need only succeed for one distribution on unlabeled examples while earlier weak-to-strong boosting theorems usually rely on the ability of the weak learner to succeed under arbitrary (or smooth) distributions. 

Instead of modifying the marginal distribution over the samples, the boosting algorithm modifies the distribution on the label of each example, usually by a rule that looks like: ``with probability $w_i$ set $\Tilde{y_i} = y_i$ otherwise, set $\Tilde{y_i} \in \{-1, 1\}$ randomly.'' \cite{kanade2009:potential} give the first such boosting algorithm then \cite{feldman2009:distribution} improve and simplify their construction. In both cases, they have similar guarantees to classical distribution-independent boosting algorithms: $O(1/\gamma^2)$ calls to the weak learner and running time $\poly(n, 1/\gamma, 1/\eps)$.

\cite{feldman2009:distribution} remark that outputting a label for $x$ with a certain expectation instead of its actual value reduces the contribution of the correlation on $x$ in the same way as regular boosting algorithms modify the weight of point $x$ to reduce or increase its contribution. In fact, they show that their distribution-specific agnostic boosting algorithm can be turned into an optimally smooth boosting algorithm


\paragraph{Jackson's DNF learning algorithm.}

==> HardcoreCircuits.tex <==
\gray{ \section{Tightness of the hardcore theorem for circuits}
Before stating the hardcore theorem, we recall the definition of a $\delta$-density distribution.
\begin{definition}[$\delta$-density distribution]
    A distribution $H$ over $\bits^n$ is a $\delta$-density distribution for $\delta>0$ if for all $x\in\bits^n$, $\Pr_{\bx\sim H}[\bx=x]\le \frac{1}{\delta 2^{n}}$. 
\end{definition}

\begin{theorem}[Impagliazzo's hardcore theorem]
    For any function $F:\bits^N \to \bits$, suppose that for size parameter $s$ and accuracy parameter $\delta$, for all circuits $C$ of size $s$,
$$\Prx_{\bx \sim \bits^N}[F(\bx) = C(\bx)] \leq 1-\delta.$$
Then, there is a hardcore set $H$ of size $\Omega(\delta 2^n)$ such that, for every circuit $C'$ of size at most $s' \le O(\frac{s\eps^2}{\log(1/\delta)})$ ,
$$\Prx_{\bx \sim H}[F(\bx) = C'(\bx)] \leq 1/2 + \eps.$$
\end{theorem} 

One unsatisfying part of the hardcore theorem is that $s'$ is \emph{smaller} than $s$, meaning the hardcore set is only hard against a weaker class (smaller circuits). Here, we show that this is necessary, and that the above dependence on $\eps$ is optimal (for constant $\delta$).

\begin{theorem}[Tightness of the hardcore theorem]
\label{thm:tight-circuits}
For any sufficiently large $s\in \N$, $\eps>0$ with $s\ge 1/\eps^4$, and $N\ge\Omega(\eps^{-2}\log s)$, there is a function $F:\bits^N\to\bits$ such that
\begin{enumerate}
    \item  For all circuits $C$ of size $s$,
	$$\Prx_{\bx \sim \bits^N}[F(\bx) = C(\bx)] \leq 0.99.$$
 \item  For all constant density $H$,\footnote{The constant here will affect that constant hidden in $N\ge \Omega(\eps^{-2}\log s)$.} there is a circuit $C'$ of size $s' \leq O(s\eps^2)$ such that,
	$$\Prx_{\bx \sim H}[F(\bx) = C'(\bx)] \geq 1/2 + \eps.$$
\end{enumerate}
\end{theorem}
} 
\lnote{I assume this stuff will be moved into the intro.}


% \begin{theorem}[Tightness of the hardcore theorem]
% \label{thm:tight-circuits}
% For any $s, \eps$ and $N \geq \frac{\log s}{\eps^2}$, there is a function $F:\bits^N \to \bits$ such that,
% \begin{enumerate}
%     \item  For all circuits $C$ of size $s$,
% 	$$\Prx_{\bx \sim \bits^N}[F(\bx) = C(\bx)] \leq 0.99.$$
%  \item For any $H$ of size $\geq 0.0001 \cdot 2^N$, there is a circuit $C'$ of size $s' \leq O(s\eps^2)$ such that,
% 	$$\Prx_{\bx \sim H}[F(\bx) = C'(\bx)] \geq 1/2 + \eps.$$
% \end{enumerate}
% \end{theorem}


% \subsection{Construction}
% \label{sec:impagliazzo-construction}
% I'm going to be loose with the constants and floor/ceilings in this analysis. Let $k = 1/\eps^2$ and set $n$ so that $s = 2^n/n$. We split the $N$ input bits into $k$ blocks each containing $n$ bits (and ignore the remaining bits). Then, we're going to set $f_1, \ldots, f_k:\bits^n \to \bits$ to each be \emph{balanced} functions, meaning
% $$\Ex_{\bx \sim \bits^n}[f_i] = 0 \quad\quad\text{for all }i \in [k].$$
% and we set
% $$F(X) = \Maj(f_1(x^{(1)}), \ldots, f_k(x^{(k)}))$$
% where $X \in \bits^{N}$ is split into $x^{(1)}, \ldots, x^{(k)}$. Note that this requires $N \geq nk$. Based on how we set $n$, it will be approximately $\log(s)$, which gives the bound on $N$ in the theorem statement.

% Our argument will show that point (2) of the \Cref{thm:tight-circuits} holds no matter how we choose $f_1, \ldots, f_k$, and point (1) holds for most choices of $f_1, \ldots, f_k$.

% \subsection{$F$ is mildly easy}

% We'll argue that, for \emph{any} choices of $f_1, \ldots, f_k$ and any set $H$ of size $\geq 0.0001 \cdot 2^n$, there is a circuit $C'$ of size $\leq s'$ such that. We give a randomized strategy that works for any choice of $H$, which can easily be derandomized for any particular choice of $H$. The strategy for $\bC'$ is to choose a random $\bi \in [k]$ and output $f_{\bi}(x^{(\bi)})$. This indeed takes size at most $s$, since any function on $n$ bits can be computed using a circuit of size $2^n/n$.

% Now fix any choice of $H$. For notational convenience, we use $\by \in \bits^k$ as the random variable indicating the output of $f_1(\bx^{(1)}), \ldots, f_k(\bx^{(k)}))$ on a random input $\bx \sim H$. Then, the success probability of $f_{\bi}(x^{(i)})$ is,

% \begin{align*}
% 	\Prx_{\by, \bi}\bracket*{\by_{\bi} = \Ind\bracket*{\sum_{i = 1}^k \by_i}} &= 1/2 + \Ex_{\by}\bracket*{\abs*{\sum_{i \in [k]} \by_i}}/(2k).
% \end{align*}

%  If we picked $X$ uniformly from all of $\bits^N$, the distribution of $\by$ would be uniform over $\bits^k$ (since each $f_i$ is balanced and the blocks are independent). The probability that $|\by_1 + \cdots + \by_k| \leq \sqrt{k}/10000$ would be a tiny constant probability. So, if $H$ has a constant fraction of the mass, the expectation of  $|\by_1 + \cdots + \by_k|$ under $H$ will be $\Omega(\sqrt{k})$. This means our strategy has accuracy $1/2 + \Omega(1/\sqrt{k})$.

%  \subsection{$F$ is mildly hard}

%  We'll say a circuit $C: \bits^{N} \to \bits$ is ``good" for a particular choice of $F = \Maj(f_1, \ldots, f_k)$ if
% $$\Prx_{\bx \sim \bits^N}[F(\bx) = C(\bx)]> 0.99.$$
% \begin{lemma}
%  Any function $C: \bits^N \to \bits$ is good for at most $2^{0.9 \cdot k 2^n}$ choices of $F = \Maj(f_1, \ldots, f_k)$.
%  \end{lemma}

% By a standard counting argument (there are at most $s^{O(s)}$ circuits of size-$s$), the above Lemma implies there exists some choice of $F$ such that all circuits $C$ of size $s$ have accuracy at most $0.99$ w.r.t $F$, proving the desired theorem.

% For this proof, fix two $F = \Maj(f_1, \ldots, f_k)$ and $F' = \Maj(f_1', \ldots, f_k')$ for which $C$ is good. By union bound,
% $$\Pr_{\bX \sim \bits^N}[F(\bX) = F'(\bX)] \geq 0.98.$$
% Let $\by$ and $\by'$ each in $\bits^k$ be the outputs of $f_1, \ldots, f_k$ and $f_1', \ldots, f_k'$ respectively on a uniform $\bX \sim \bits^N$.  Let $\delta_i = \Pr_{\bx \sim \bits^n}[f_i(\bx) \neq f_i'(\bx)]$. 

% \emph{more todo}




